Ergodic properties of linked-twist maps

We study a class of homeomorphisms of surfaces collectively known as linked-twist maps. We introduce an abstract definition which enables us to give a precise characterisation of a property observed by other authors, namely that such maps fall into one of two classes termed co- and counter-twisting. We single out three specific linked-twist maps, one each on the two-torus, in the plane and on the two-sphere and for each prove a theorem concerning its ergodic properties with respect to the invariant Lebesgue measure. For the map on the torus we prove that there is an invariant, zero-measure Cantor set on which the dynamics are topologically conjugate to a full shift on the space of symbol sequences. Such features are commonly known as topological horseshoes. For the map in the plane we prove that there is a set of full measure on which the dynamics are measure-theoretically isomorphic to a full shift on the space of symbol sequences. This is commonly known as the Bernoulli property and verifies, under certain conditions, a conjecture of Wojtkowski's. We introduce the map on the sphere and prove that it too has the Bernoulli property. We conclude with some conjectures, drawn from our experience, concerning how one might extend the results we have for specific linked-twist maps to the abstract linked-twist maps we have defined.

==> input/intro.tex <==
\renewcommand{\thechapter}{\Alph{chapter}}
\setcounter{chapter}{0}
\chapter*{Introduction} 
\addcontentsline{toc}{chapter}{Introduction} 
\chaptermark{Introduction}
\setcounter{equation}{0}
\setcounter{figure}{0}
\label{intro}
\renewcommand{\thechapter}{\arabic{chapter}}

Introduction text
